FastQuery: Communication-efficient Embedding Table Query for Private LLM Inference

With the fast evolution of large language models (LLMs), privacy concerns with user queries arise as they may contain sensitive information. Private inference based on homomorphic encryption (HE) has been proposed to protect user query privacy. However, a private embedding table query has to be formulated as a HE-based matrix-vector multiplication problem and suffers from enormous computation and communication overhead. We observe the overhead mainly comes from the neglect of 1) the one-hot nature of user queries and 2) the robustness of the embedding table to low bit-width quantization noise. Hence, in this paper, we propose a private embedding table query optimization framework, dubbed FastQuery. FastQuery features a communication-aware embedding table quantization algorithm and a one-hot-aware dense packing algorithm to simultaneously reduce both the computation and communication costs. Compared to prior-art HE-based frameworks, e.g., Cheetah, Iron, and Bumblebee, FastQuery achieves more than $4.3\times$, $2.7\times$, $1.3\times$ latency reduction, respectively and more than $75.7\times$, $60.2\times$, $20.2\times$ communication reduction, respectively, on both LLAMA-7B and LLAMA-30B.

==> docs/7-Discussion.tex <==
\section{DISCUSSION}
\paragraph{Lower bound of the plaintext module $p$}
The lower bound of $p$ is influenced by cryptographic requirements. On the one hand, if we use batch encoding in Microsoft SEAL~\cite{sealcrypto}, $p$ must be a prime and satisfies $p\mod 2^n=1$ and we cannot find a suitable prime under low bit-width. On the other hand, we experimentally find if the bit-width is less than 13 bits, it cannot guarantee HE computation correctness. Additionally, in practice, one would not choose a particularly low $p$ as it requires flexibility to support multiple layers and networks.

\paragraph{Memory reduction of~\method} In HE-based private inference, memory cost mainly depends on the number of plaintext and ciphertext of input, weight, and output. Hence,~\method~also reduces the memory requirements since it significantly reduces the number of polynomials. However, memory-efficient HE-based private inference is a timely and important topic and will be part of our future work.


==> docs/outline.tex <==
\textbf{Outlines:}
\begin{itemize}
    \item Motivation: the first step of large language models (LLMs) inference is to query the embedding table, which is formulated as a matrix-vector multiplication problem during private inference. The basic steps for private embedding table query include:
    \begin{itemize}
        \item Generate a one-hot vector based on the token ID.
        \item Compute the multiplication between the embedding weight and the vector.
        \item Post-processing: align bit precisions, scales, or dimensions
    \end{itemize}
    
    \item However, due to the large vocabulary size, the latency and communication for private embedding table query is very high, accounting for XXX\% of a Transformer block. \ml{Need to emphasize total communication is the most important metric. Need to make a comparison between the communication/latency of embedding table query and one transformer layer for both regular and private inference.}
    
    \item Review existing matrix-vector multiplication methods, including Cheetah, Iron, and BubbleBee, as well as PIR methods, including FastPIR, INSPIRE, SqueezePIR, etc. Need to highlight their pros and cons.
    
    \item Existing methods are not efficient enough as they usually ignore the following properties for embedding table query:
    \begin{itemize}
        \item Matrix-vector multiplication methods: HE is leveraged to generate the help data, which loses the property of the query as a one-hot vector, i.e., only one element of the query is 1 while all the other elements are 0s. With the property, for 
        % \item Matrix-vector multiplication methods: ignore the query is a one-hot vector, i.e., only one element of the query is 1 while all the other elements are 0s. This indicates for the 
        the SIMD encoding, no rotations are needed for accumulation while for both SIMD and coefficient encoding, the accumulation bit precision is the same as the weight bit precision.
        \item PIR methods: ignore the key characteristics of the LLM embedding matrix, e.g., low precision, token frequency, etc.
        \item The input dimension is usually much higher compared to the output dimension, while without PackLWE, the packing density of the output is much lower.
        \ml{@chenqi, @tianshi, profile the input and output communication for different baselines, including Iron, Addre, and CHAM.}
        % \item Other observations: the imbalance between input and output communication \ml{Need to verify}
    \end{itemize}

    \item To improve the efficiency for embedding table query:
    \begin{itemize}
        \item Analyze and compare different encoding schemes (both theoretically and experimentally)
        \item How to reduce the input communication: hierarchical query? \ml{@chenqi, @tianshi needs to quantify the impact on communication and computation both theoretically and experimentally.}
        \item How to reduce the output communication: PackLWE \ml{What is the difference between rotations in SIMD encoding and automorphisms in coefficient encoding?}
        \item How to reduce the computation overhead: packing more elements within one co-efficient, embedding table quantization with per-column/per-group quantization, perplexity-guided mixed precision strategy \ml{@zebin}
    \end{itemize}

    \item Experimental results: \ml{@chenqi, @tianshi think of experimental results for the paper}
    \begin{itemize}
        \item Comparison of different embedding table quantization methods for different LLMs, including LLAMA, BERT, etc.
        \item Communication and latency comparison of different methods.
    \end{itemize}

    \item Note
    \begin{itemize}
        \item Computation (including both multiplication and automorphism) can be accelerated with GPU: https://github.com/lightbulb128/troy
        \item \ml{Think about how to reduce the communication for the output projection layer}
    \end{itemize}
\end{itemize}

\noindent\rule[0.5ex]{\linewidth}{1pt}

Notations:
\begin{itemize}
    \item Embedding table: $W \in \R^{m \times n}$, where $m$ denotes 
        the embedding table size and $n$ denotes the embedding dimension
    \item Query: $X$ is an one-hot encoded vector of dimension $m$
    \item HE parameters: $N, q, p$ denote the number of slots, ciphertext
        modulus, and plaintext modulus, respectively.
    \item The outputs of the protocol are secret shares of the query output.
\end{itemize}

How to compute the embedding table query with MPC/HE:
\begin{itemize}
    \item Baseline (Iron) \cite{hao2022iron}: 
    \begin{itemize}
        \item Matrix multiplications with co-efficient packing
    \end{itemize}
    
    \item Bubblebee: 
    \begin{itemize}
        \item Matrix multiplications with co-efficient packing
        \item Ciphertext interleaving/repacking (require rotations)
    \end{itemize}
    
    \item FastPIR \cite{ahmad2021addra}:
    \begin{itemize}
        \item Matrix multiplications with SIMD packing
        \item Ciphertext repacking (require rotations)
        \item Packing multiple low-precision values into a single slot
    \end{itemize}
    
    \item INSPIRE \cite{lin2022inspire}: 
    \begin{itemize}
        \item Divide a query into group query and block query on top of FastPIR
    \end{itemize}

    \item SqueezePIR \cite{liang2023spg}:
    \begin{itemize}
        \item Leverage low-rank approximation for embedding table compression
    \end{itemize}
\end{itemize}

\begin{table}[!tb]
\caption{Computation costs include both polynomial multiplications and 
rotations. Communication costs include both input and output polynomial 
transfer communication.}
\label{tab:comp}
\centering
\begin{tabular}{c|ccc|cc}
\toprule
\multirow{2}{*}{Protocol} & \multicolumn{3}{c|}{Computation}   & \multicolumn{2}{c}{Communication} \\
\cline{2-6}
                         & PT-CT Mul & CT-CT Mul & Rotations/Automorphism & Input           & Output          \\
\midrule
Baseline                 &           &           &           &                 &                 \\
Bubblebee                &           &           &           &                 &                 \\
FastPIR                  &           &           &           &                 &                 \\
INSPIRE                  &           &           &           &                 &                 \\                        
SqueezePIR               &           &           &           &                 &                 \\                        
\bottomrule
\end{tabular}
\end{table}

Optimizations:
\begin{itemize}
    \item Token frequency-aware adaptive embedding compression:
    \begin{itemize}
        \item Cluster the tokens in the embedding table based on the token frequency
        \item Apply more aggressive compression (e.g., low-rank approximation or
            low precision compression or both) to less frequent clusters
        \item To determine which cluster the token belongs to, can leverage the
            protocol for one-hot vector generation from PUMA
        \item The same protocol can be applied for Mixture-of-Expert?
    \end{itemize}
\end{itemize}

==> texlib/acm_setting.tex <==
% =============================================================
%            settign for ACM format paper
%
%   Author      : Bei Yu
%   Last Update : 12/2014
% =============================================================

\settopmatter{printacmref=false}          % no ACM Reference Format
\fancyhead{}                              % no header

% ==== page margin settings
\geometry{twoside=true, head=13pt,
	paperwidth=8.5in, paperheight=11in,
	includeheadfoot, columnsep=2pc,
	top=35pt, bottom=45pt, 
    left=40pt, right=40pt, 
    %inner=54pt, outer=54pt,
	marginparwidth=2pc,heightrounded
}%
%\geometry{twoside=true, head=13pt,
%paperwidth=8.5in, paperheight=11in,
%includeheadfoot, columnsep=2pc,
%top=57pt, bottom=73pt, inner=54pt, outer=54pt,
%marginparwidth=2pc,heightrounded
%}%
\iffalse
\textfloatsep          = 12pt plus 1pt minus 7pt            % set space between figure and text
\floatsep              = 5pt plus 1pt minus 7pt
\fi
%\intextsep             = 0pt plus 1pt minus 7pt           % set space above and below the texts
%\dbltextfloatsep       = 0pt plus 1pt minus 7pt
%\dblfloatsep           = 0pt plus 1pt minus 7pt
%\abovedisplayskip      = 0pt plus 1pt minus 7pt           % set space around equations
%\belowdisplayskip      = 0pt plus 1pt minus 7pt
%\abovedisplayshortskip = 0pt plus 1pt minus 7pt
%\belowdisplayshortskip = 0pt plus 1pt minus 7pt

% ==== Packages
\usepackage{graphicx}
\usepackage{amsmath}
\let\Bbbk\relax
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{comment}
\usepackage[subrefformat=parens,labelformat=parens]{subfig}
\captionsetup[subfigure]{labelformat=simple}               % avoid "double brackets" in sub-figure caption
\renewcommand\thesubfigure{(\alph{subfigure})}             % "Fig.~1b"-->"Fig.1(b)"
\usepackage{bm}
\usepackage{multirow}
\usepackage{threeparttable,booktabs}
\usepackage{tikz}
\usepackage{balance}
\usepackage{courier}                                       % courier font, used in \texttt
\usepackage{cleveref}                                      % smart citation
\usepackage[mathcal]{eucal}
%\usepackage[]{algpseudocode}                               % algorithm package
\usepackage[noend]{algpseudocode}
\algrenewcommand\textproc{\texttt}
\makeatletter\let\float@addtolists\relax\makeatother
\usepackage{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:} }       % Use Input in the format of Algorithm
\renewcommand{\algorithmicensure} {\textbf{Output:}}       % Use Output in the format of Algorithm
\usepackage{filecontents}                                  % support to pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
\usepackage{siunitx}


\sisetup{product-units = single}
% ==== Local new commands
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\renewcommand{\vec}[1]{\boldsymbol{#1}} 
\newcommand{\m}[1]{\mathbf{#1}}
\newcommand{\mx}{\m{x}}
\newcommand{\my}{\m{y}}
\newcommand{\mz}{\m{z}}
\DeclareMathOperator*{\argmin}{argmin}

\theoremstyle{plain}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}

\theoremstyle{definition}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{myproblem}{\textbf{Problem}}



% ==== spacing control on caption
\usepackage[skip=1pt]{caption}            % set space between figure and caption
\setlength{\belowcaptionskip}{-1.0mm}
\captionsetup[table]{aboveskip=5pt}       % reduce space around table caption
\captionsetup[table]{belowskip=2pt}


==> texlib/ieee_setting.tex <==
% =============================================================
%            setting for IEEE format paper
%
%   Author      : Bei Yu
%   Last Update : 06/2015
% =============================================================


%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}    % new algorithm package
\usepackage{algorithm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{subfigure}
\usepackage{graphicx}         % include pdf figures
\usepackage{color}
\usepackage{cite}             % more citations in one bracket
\usepackage{comment}          % use comment
\usepackage{soul}             % use highlight command \hl{}
\soulregister\cite7
\soulregister\ref7
\soulregister\pageref7
\usepackage{amsthm}
\usepackage{etoolbox}         % commands \newtoggle, \toggletrue, \iftoggle
\usepackage{url}
\usepackage{nth}              % nth command
\usepackage{bm}               % bm command


\newtheorem{myproblem}{\textbf{Problem}}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}
\newtheorem{myapplication}{\textbf{Application}}
\newtheorem{myconjecture}{Conjecture}


% long line in algorithm
% e.g.: \Statex[4] ...;
\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][3]{%
  \setlength\@tempdima{\algorithmicindent}%
  \OldStatex\hskip\dimexpr#1\@tempdima\relax
}
\makeatother


% ==== Logs:
%
%  06/2015: clean IEEEtranBSTCTL commands
%  11/2014: \solregister, to support highlight to mybox, definition, and citations
%  10/2014: add package "authblk" & "bm"
%  09/2014: "problem" => "myproblem"
%  07/2014: introduce \Statex[] for lone algorithmic statement
%  05/2014: new package {soul} to use highlight command \hl{}
%




==> texlib/poster_setting.tex <==
% ============================================================
%             Beamer poster setting file
%
%   Author      : Bei Yu
%   last Update : 06/2014
% ============================================================

% additional settings
\setbeamerfont{itemize}{size=\normalsize}
\setbeamerfont{itemize/enumerate body}{size=\normalsize}
\setbeamerfont{itemize/enumerate subbody}{size=\normalsize}


% block width setting
\newenvironment<>{varblock}[2][\textwidth]{%
  \setlength{\textwidth}{#1}
  \setbeamercolor{block title}{fg=white,bg=blue!20!green}
  %\setbeamercolor{block body}{fg=black,bg=olive!50}
  \setbeamercolor{block body}{fg=black,bg=blue!10}
  \begin{actionenv}#3%
  \def\insertblocktitle{#2}%
  \par%
  \usebeamertemplate{block begin}}
  {
    \par%
    \usebeamertemplate{block end}%
    \end{actionenv}
  }


% abbreviations
\usepackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{{e.g}\onedot} \def\Eg{{E.g}\onedot}
\def\ie{{i.e}\onedot} \def\Ie{{I.e}\onedot}
\def\cf{{c.f}\onedot} \def\Cf{{C.f}\onedot}
\def\etc{{etc}\onedot}
\def\vs{{vs}\onedot}
\def\wrt{w.r.t\onedot}
\def\dof{d.o.f\onedot}
\def\etal{{et al}\onedot}
\makeatother


% === including packages
\usepackage{bm}
\usepackage{xcolor}
\usepackage{colortbl}
\usepackage{times}
\usepackage{amsmath,amsthm, amssymb, latexsym}
\usepackage{exscale}
\usepackage{subfigure}
\usepackage{multirow}
\usepackage{comment}
\usepackage{booktabs, array}
\usepackage[english]{babel}
\usepackage[latin1]{inputenc}
\usepackage[orientation=landscape,size=custom,width=200,height=230,scale=1.9]{beamerposter}
\listfiles

% =====  algorithm setting
%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}
\usepackage{algorithm}
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}  % Use Input in the format of Algorithm
%\renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm

% ==== Log
%
%  05/2014: preliminary results show that pgf library is NOT good for poster
%


